Observing the polarized cosmic microwave background from the Earth: scanning strategy and polarimeters test for the LSPE/STRIP instrument

Detecting B-mode polarization anisotropies on large angular scales in the CMB polarization pattern is one of the major challenges in modern observational cosmology since it would give us an important evidence in favor of the inflationary paradigm and would shed light on the physics of the very early Universe. Multi-frequency observations are required to disentangle the very weak CMB signal from diffuse polarized foregrounds originating by radiative processes in our galaxy. The "Large Scale Polarization Explorer" (LSPE) is an experiment that aims to constrain the ratio between the amplitudes of tensor and scalar modes and to study the polarized emission of the Milky Way. LSPE is composed of two instruments: SWIPE, a stratospheric balloon operating at 140, 210 and 240 GHz that will fly for two weeks in the Northern Hemisphere during the polar night of 2021, and STRIP, a ground-based telescope that will start to take data in early 2021 from the "Observatorio del Teide" in Tenerife observing the sky at 43 GHz and 95 GHz. In my thesis, I show the results of the unit-level tests campaign on the STRIP detectors that took place at "Universit\`a degli Studi di Milano Bicocca" from September 2017 to July 2018, and I present the code I developed and the simulations I performed to study the STRIP scanning strategy. During the unit-level tests, more than 800 tests on 68 polarimeters have been performed in order to select the 55 with the best performance in terms of central frequencies, bandwidths, noise temperatures, white noise levels, slopes and knee frequencies. The STRIP scanning strategy is based on spinning the telescope around the azimuth axis with constant elevation in order to overlap the SWIPE coverage maintaining a sensitivity of 1.6 {\mu}K (on average) per sky pixels of 1{\deg}. Individual sources will be periodically observed both for calibration and study purposes.

==> Ackno.tex <==
\chapter*{Acknowledgments}
\thispagestyle{plain}

  


==> PartIII.tex <==
\part*{Part III\vspace{0.5cm}\\Measuring the Earth's atmosphere from the ground}





==> chap7.tex <==
\chapter{Impact of the Earth's atmosphere on the CMB polarization ground-based experiments}
\label{Chap:7}
\thispagestyle{plain}


\section{Earth’s atmosphere properties}
\section{Impact of the atmosphere on the signal}
\section{Polarized atmospheric signal}
\subsection{Zeeman splitting of oxygen}
\subsection{Troposhperic ice clouds}
\section{Prescriptions to disentangle the atmospheric signal}
\subsection{General prescriptions}
\subsection{The STRIP case}


==> chap8.tex <==
\chapter{Simulating the measurement of the atmosphere temperature with STRIP}
\label{Chap:8}
\thispagestyle{plain}


\section{Impact on the instrumental sensitivity: the secant law}
\subsection{Antenna temperature definition}
\section{Monte Carlo simulations}
\subsection{Model assumptions}
\section{Results}
\subsection{Elevation scans}
\subsection{Nominal }
\section{Future directions}

